RealTalk: Real-time and Realistic Audio-driven Face Generation with 3D Facial Prior-guided Identity Alignment Network

Person-generic audio-driven face generation is a challenging task in computer vision. Previous methods have achieved remarkable progress in audio-visual synchronization, but there is still a significant gap between current results and practical applications. The challenges are two-fold: 1) Preserving unique individual traits for achieving high-precision lip synchronization. 2) Generating high-quality facial renderings in real-time performance. In this paper, we propose a novel generalized audio-driven framework RealTalk, which consists of an audio-to-expression transformer and a high-fidelity expression-to-face renderer. In the first component, we consider both identity and intra-personal variation features related to speaking lip movements. By incorporating cross-modal attention on the enriched facial priors, we can effectively align lip movements with audio, thus attaining greater precision in expression prediction. In the second component, we design a lightweight facial identity alignment (FIA) module which includes a lip-shape control structure and a face texture reference structure. This novel design allows us to generate fine details in real-time, without depending on sophisticated and inefficient feature alignment modules. Our experimental results, both quantitative and qualitative, on public datasets demonstrate the clear advantages of our method in terms of lip-speech synchronization and generation quality. Furthermore, our method is efficient and requires fewer computational resources, making it well-suited to meet the needs of practical applications.

==> table/abl_scale.tex <==
\begin{tabular}{@{}clllll@{}}
\toprule
\multicolumn{1}{l}{Num of Blocks} & FID                       & LPIPS                               & SSIM                                & Speed                     & Para.                         \\ \midrule
1                                 &                           &                                     &                                     &                           &                               \\
2                                 & \multicolumn{1}{r}{\textbf{12.73}} & \multicolumn{1}{r}{\textbf{0.0916}} & \multicolumn{1}{r}{\textbf{0.9361}} & \multicolumn{1}{r}{30.82} & \multicolumn{1}{r}{69.24} \\
3                                 &                           &                                     &                                     &                           &                               \\ \bottomrule
\end{tabular}

==> table/rebuttal/hdtf.tex <==
\setlength{\tabcolsep}{14pt}
\begin{tabular}{@{}llllll@{}}
\toprule
Metric & M-LMD   $\downarrow$       & F-LMD    $\downarrow$       & FID   $\downarrow$  & LPIPS $\downarrow$  & SSIM      $\uparrow$    \\ \midrule
DINet  & 15.36        & 5.185          & 12.94  & 0.0975   & 0.9327    \\
IP-LAP & 10.20        & 4.658          & 9.490     &   0.1101 &   0.9416    \\
Ours   & \textbf{9.966} & \textbf{4.207} & \textbf{6.065} &  \textbf{0.0820}  &  \textbf{0.9418} \\ \bottomrule
\end{tabular}

==> table/rebuttal/lmd.tex <==
% \setlength{\tabcolsep}{8pt}
\begin{tabular}{@{}lllllll@{}}
\toprule
Metric & Wav2Lip & PC-AVS & TalkLip & DINet & IP-LAP & Ours           \\ \midrule
M-LMD $\downarrow$ & 15.88   & 22.09  & 31.83   & 24.58 & 14.45  & \textbf{11.02} ($\downarrow$3.43) \\
F-LMD $\downarrow$ & 5.826   & 24.67  & 14.06   & 15.61 & 6.292  & \textbf{4.923} ($\downarrow$0.90) \\ \bottomrule
\end{tabular}


% \setlength{\tabcolsep}{10pt}
% \begin{tabular}{@{}lllll@{}}
% \toprule
% Dataset & \multicolumn{2}{c}{Voxceleb1}      & \multicolumn{2}{c}{MEAD}           \\ 
% Metric  & M-LMD  $\downarrow$          & F-LMD    $\downarrow$       & M-LMD    $\downarrow$        & F-LMD   $\downarrow$        \\ \midrule
% % Wav2Lip & 15.8769          & 5.8262          & 29.0242          & 6.6114          \\
% % PC-AVS  & 22.0889          & 24.6647         & 26.7314          & 18.35           \\
% % TalkLip & 31.8301          & 14.061          & 34.1059          & 9.5925          \\
% DINet   & 24.58          & 15.61          & 38.14          & 5.828         \\
% IP-LAP  & 14.45          & 6.292          & 18.68          & 5.271          \\
% Ours    & \textbf{11.02} & \textbf{4.923} & \textbf{18.65} & \textbf{5.029} \\ \bottomrule
% \end{tabular}
